How Can Human Values Be Addressed in Agile Methods? A Case Study on SAFe

Agile methods are predominantly focused on delivering business values. But can Agile methods be adapted to effectively address and deliver human values such as social justice, privacy, and sustainability in the software they produce? Human values are what an individual or a society considers important in life. Ignoring these human values in software can pose difficulties or risks for all stakeholders (e.g., user dissatisfaction, reputation damage, financial loss). To answer this question, we selected the Scaled Agile Framework (SAFe), one of the most commonly used Agile methods in the industry, and conducted a qualitative case study to identify possible intervention points within SAFe that are the most natural to address and integrate human values in software. We present five high-level empirically-justified sets of interventions in SAFe: artefacts, roles, ceremonies, practices, and culture. We elaborate how some current Agile artefacts (e.g., user story), roles (e.g., product owner), ceremonies (e.g., stand-up meeting), and practices (e.g., business-facing testing) in SAFe can be modified to support the inclusion of human values in software. Further, our study suggests new and exclusive values-based artefacts (e.g., legislative requirement), ceremonies (e.g., values conversation), roles (e.g., values champion), and cultural practices (e.g., induction and hiring) to be introduced in SAFe for this purpose. Guided by our findings, we argue that existing Agile methods can account for human values in software delivery with some evolutionary adaptations.

==> Figures/FigureTex/CodingProcess.tex <==
\begin{figure*}[t]
	\centering
	\vspace{0cm}
	\includegraphics[width=1\textwidth]{Figures/CodeProcess.png}
	\vspace{-6mm}
	\caption{Test}
	\label{fig:codingproces}
\end{figure*}

==> Figures/FigureTex/Interviewee_demography.tex <==
\begin{figure*}[t]
	\centering
	\vspace{0cm}
	\includegraphics[width=1\textwidth]{Figures/FindingsSummary.PNG}
	\vspace{-6mm}
	\caption{Interviewee demography for Case 1 (red) and Case 2 (green)}
	\label{fig:demography}
\end{figure*}

==> Figures/FigureTex/Summary.tex <==
\begin{figure*}[hbt!]
	\centering
% 	\includegraphics[width=0.98\textwidth]{Figures/NewTablesImages/design.png}
% 	\vspace{-0.5cm}
	\includegraphics[width=0.98\textwidth]{Figures/Findings6.png}
% 	\vspace{-4mm}
    \caption{Findings Summary}
	\label{fig:findings}
\end{figure*}


==> Figures/FigureTex/demographics.tex <==
% \begin{table*}
% 	%\centering

%  	%\vspace{-4mm}
%     \caption{Interviewee Demographics (M: Male, F: Female, y: Year, m: Month)}
% 	\label{tbl:demography1}
% 	\includegraphics[width=0.95\textwidth]{Figures/Demographics4.png}
% \end{table*}

%\input{Tables/Demographic}

%\begin{figure*}[htb]
%	\centering
%\includegraphics[width=0.95\textwidth]{Figures/Demographics4.png}
 %	\vspace{-4mm}
  %  \caption{Interviewee Demographics (M: Male, F: Female, y: Year, m: Month)}
%	\label{fig:demography1}
%\end{figure*}


%\begin{figure*}[htb]
	%\centering
	%\includegraphics[width=0.45\linewidth]{Figures/ObservationSamall.png}
 	%\vspace{-4mm}
    %\caption{Observations}
	%\label{fig:demography}
%\end{figure*}

%\begin{figure*}[htb]
%	\centering
    %\includegraphics[width=1\textwidth]{Figures/FigureTex/DataAnaProcess.pdf}
%	\vspace{-3mm}
 %  \caption{Data analysis process using Thematic Analysis}
%	\label{fig:dataanalysis}
%\end{figure*}

% \begin{table*}
% %	\centering
% 	\caption{Examples of open coding}
% 	\label{tbl:codingexample}
%     \includegraphics[width=0.95\textwidth]{Figures/CodeExamplesV1.png}
% %	\vspace{-4mm}
% \end{table*}

%\input{Tables/CodingExamples}

%\begin{figure*}[htb]
%	\centering
 %   \includegraphics[width=0.95\textwidth]{Figures/CodeExamplesV1.png}
%	\vspace{-4mm}
 %  \caption{Examples of open coding}
%	\label{fig:codingexample}
%\end{figure*}









==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Tables/FindingSummary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{Findings Summary; * denotes new ideas emerged}
\label{tab:SummaryResults}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\textbf{Intervention point} & \textbf{SAFe Level (T - Team /P - Program)} & \textbf{Timeline} \\ \hline
\multicolumn{3}{|c|}{\textbf{Artefacts}}  \\ \hline
\textbf{User stories:}   Translators understand the business language customer representatives use but at the same time can understand the technical language used by the development team that helps to overcome the language barrier between the two groups          &  T    &     \\ \hline
\textbf{Epics:} This is a sample explanation               & T       &     \\ \hline
\textbf{Personas :} This is a sample explanation           & T       &     \\ \hline
\textbf{Journey Maps:}                                     & T       &     \\ \hline
\textbf{Non-Functional Requirements List:}                 & T       &     \\ \hline
\textbf{Checklists*:}                                     & T,P     &     \\ \hline
\textbf{Legislative Requirements*:}                         & P       &     \\ \hline
\textbf{Corporate Directives*:}                             & P       &     \\ \hline
\multicolumn{3}{|c|}{\textbf{Roles}}      \\ \hline
\textbf{Product Owner:}                                     & T       &     \\ \hline
\textbf{Business Owner:}                                    & T       &     \\ \hline
\textbf{Release Train Engineer:}                            & T       &     \\ \hline
\textbf{Value Champions*:}                                  & T       &     \\ \hline
\textbf{Value Promoters*:}                                  & T       &     \\ \hline
\textbf{Values Mentor*:}                                    & T       &     \\ \hline
\textbf{Values Translators*:}                               & T       &     \\ \hline
\textbf{Value Officers*:}                                   & T       &     \\ \hline
\textbf{Change Manager*:}                                  & T       &     \\ \hline
\multicolumn{3}{|c|}{\textbf{Ceremonies}} \\ \hline
\textbf{Daily Stand-Ups:}                                   & P       &     \\ \hline
\textbf{Inspect and Adapt and Retrospective Meetings:}      & P       &     \\ \hline
\textbf{Program Increment Planning:}                        & P       &     \\ \hline
\textbf{Kick Off:}                                          & P       &     \\ \hline
\multicolumn{3}{|c|}{\textbf{Practices}}  \\ \hline
\textbf{Testing:}                                          & T       &     \\ \hline
\textbf{Values Conversation*:}                              & T       &     \\ \hline
\multicolumn{3}{|c|}{\textbf{Culture}}    \\ \hline
\textbf{Induction and On-boarding:}                         & P       &     \\ \hline
\textbf{Leadership - Behaviour Role Modelled:}              & P       &     \\ \hline
\textbf{Collective Responsibility:}                       & P       &     \\ \hline
\end{tabular}%
}
\end{table*}

==> Tables/FindingSummary2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{Findings Summary: intervention points in SAFe to introduce human values in software \newline
\faLightbulbO: new ideas emerged;  \faEdit: modifying existing items; \faUsers: Culture; T: SAFe \textbf{Team} Level; P: SAFe  \textbf{Program} Level}
%\harsha{shouldn't we bring the legend here, aligning with other tables}} 
%\waqar{@ Arif, please remove the extra line below}
\label{tab:SummaryResultsNew2}
\vspace{-3mm}
{\renewcommand{\arraystretch}{1.3}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{p{17cm}p{0.2cm}p{0.2cm}}
\hline
\textbf{Intervention point} & \textbf{N} & \textbf{L}  \\ \hline 
\rowcolor{lightgray}\multicolumn{3}{c}{\textbf{Artefacts}} \\ \hline
\textbf{\faEdit {} User story:} state human values in the `\textit{so that}' part of a user story to capture its purpose or the bigger `why'. & Y & T   \\
%addresses user needs and goals that can be modified to state/capture a human value as the purpose or the bigger why in `\textit{so that}' part of the story. & T   \\
\textbf{\faEdit {} Epic/Feature:} state human values as high level requirements in the epic/feature definition. & Y & T   \\
%Large work items (too large to be completed by a single team in one iteration) whose description can contain values as high level requirements./epic
\textbf{\faEdit {} Persona:} state users values as higher-order goals in persona definition as potential expectations to be satisfied by the system %state users values expectations in persona definition as goals to be satisfied by the system
.& Y &T   \\
%reflects human personality and goals of a specific group of users that can be modified to capture and describe values people may hold.
\textbf{\faEdit {} User Journey Map:} describe the values of users affected by system usage when they try to achieve their goals.& Y & T   \\
%Visual descriptions of emotions a user goes through while accomplishing their goals that can be expanded to express values affected in fulfilling their goals through system use. & T   \\
\textbf{\faLightbulbO{} Checklist:} list values to be explicitly considered or addressed during development and validated through users feedback of the system.& Y & T   \\
%list values to be considered during system development/evaluation to reduce failure due to potential limits of human memory or attention and also to ensure task completeness& 
%A job-aid artefact listing values to be considered during system development/evaluation to reduce failure due to potential limits of human memory or attention and ensures task completeness. & T \& P   \\
\textbf{\faLightbulbO{} Legislative Requirement:} incorporate regulatory guidelines %or standards
into development processes to avoid violations of privacy/security etc.& Y & P   \\
%Regulations from government and consumer right protection bodies to ensure human values like privacy/security etc. are not violated by software.& P   \\
\textbf{\faLightbulbO{} Corporate Directive:} introduce corporate directives encouraging values consideration in software beyond security/privacy.& Y &P   \\ \hline
\rowcolor{lightgray}\multicolumn{3}{c}{\textbf{Roles}} \\ \hline
\textbf{\faEdit {} Product Owners:} optimise business value by ensuring human values are also addressed in the system delivered.& Y & T   \\
%optimises business value creation in the product and also ensure human values are delivered in the system. & T   \\
\textbf{\faEdit {} Business Owners:} provide inputs on what satisfies users values expectations to maximise value (creation) for stakeholders.& Y & T   \\
%determines what maximises value creation for the stakeholders and also provides inputs as to what satisfies stakeholders' human value expectations. & T   \\
\textbf{\faEdit {} Release Train Engineer:} ensure alignment between the Agile process and human values is never derailed during development.& Y & T   \\
%\textbf{\faEdit {} Release Train Engineer:} shepherds the delivery teams to ensure the alignment with (agile and) human values is never derailed throughout software development life-cycle. & T   \\
\textbf{\faLightbulbO{} Values Champions:} actively advocate for values inclusion and keep it alive in people's minds to ensure success.& Y &T   \\
\textbf{\faLightbulbO{} Values Mentors:} guide development teams and encourage continuous adherence to values while developing software.& Y &T   \\
\textbf{\faLightbulbO{} Values Translators:} communicate values concepts in a terminology understandable for the development teams.& Y &T   \\
\textbf{\faLightbulbO{} Values Promoters:} advocate for inclusion of human values in software and help overcome barriers encountered.& Y &T   \\
\textbf{\faLightbulbO{} Values Officers:} answer values-specific questions and ensure values related directives and guidelines are adhered to.& Y &T   \\ \hline
\rowcolor{lightgray}\multicolumn{3}{c}{\textbf{Ceremonies}} \\ \hline
\textbf{\faEdit {} Stand-ups:} align development work with its `higher propose'; reflect on 'how \textit{this} work upholds \textit{that} human value'.& Y &P   \\
%can go beyond sharing work progress to align the development work with it's `higher propose' through questions like 'how is the work you are doing today upholding that value'& P   \\
\textbf{\faEdit {} Inspect and Adapt:} reflect on current practices and propose new ways to embed human values in software. & Y &P  \\
%facilitate  review  team  practices  to  identify  was  for  improvement  to  be  expanded  to  review activities and practices to embed values
\textbf{\faEdit {} PI Planning:} align organisational vision with stakeholder values to plan software delivery accordingly. & Y &P   \\
%help align all the teams to a shared vision to be modified to align  stakeholder value expectations with development organisation's values. & P   \\
\textbf{\faEdit {} \textbf{Kick Offs:}} allow key stakeholders to define major human values objectives for the entire project. & Y & P   \\
\faLightbulbO{} \textbf{Values Conversations:} prioritise human values and contemplate the implications of values breaches by software use.& Y &T 
\\ \hline
%allow key stakeholders to define major project goals and can also be used to define values objectives for the entire project. & P & 
\rowcolor{lightgray}\multicolumn{3}{c}{\textbf{Practices}} \\ \hline
\textbf{\faEdit {} Business Facing Testing:} seek user feedback beyond usability, functionality to capture users experiences of their values expectations. & Y &T   \\ \hline
%seeking feedback beyond usability, functionality and performance to capture users experiences of their values expectations. & T   \\
%\faLightbulbO{} \textbf{Values Conversations:} prioritise human values and contemplate the implications of values breaches by software use.& T   
%focus on discussing human values, contemplating the implications of values breaches and identifying ways to embed them into software delivery.& T   
%\\ \hline
\rowcolor{lightgray}\multicolumn{3}{c}{\textbf{ Culture}} \\ \hline
\textbf{\faUsers {} Hiring/Induction:} %hire people with values aligned to the organisational values and foster a values-driven culture \waqar{through awareness and training}. 
Prioritise hiring for values alignment;  foster a culture of recognition for behaviour exemplifying desired values. & Y &P 
 \\
\textbf{\faUsers {} Leadership:} role-model values-based thinking and action as an example behaviour for the (development) teams to follow.& Y &P   \\
%that rubs off values-based thinking and action onto the development teams by role modelling it as a behaviour rather than seeking compliance through command and control.& P   \\
\textbf{\faUsers {} Collective Responsibility:} share responsibility to address human values throughout the development life cycle.
& Y & P  \\ \hline
%\multicolumn{2}{c}{\faLightbulbO{}: new ideas emerged; \faEdit{}: modifying existing items; \faUsers{}: Culture; T: SAFe \textbf{Team} Level; P: SAFe \textbf{Program} Level} \\
\end{tabular}%
} \quad
\end{table*}


==> Tables/FindingSummary_mod.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{Findings Summary: intervention points in SAFe to introduce human values in software}
\label{tab:SummaryResults}
\vspace{-3mm}
{\renewcommand{\arraystretch}{1.5}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{p{15cm}cl}
\hline
\textbf{Intervention point} & \textbf{ Level} & \textbf{When} \\ \hline 
\multicolumn{3}{c}{\textbf{Artefacts}} \\ \hline
\textbf{\faEdit {} User story:} state human values in the `\textit{so that}' part of a user story to capture its purpose or bigger `why'. & T &  \\
%addresses user needs and goals that can be modified to state/capture a human value as the purpose or the bigger why in `\textit{so that}' part of the story. & T &  \\
\textbf{\faEdit {} Epic/Feature:} state human values as high level requirements in the epic/feature definition. & T &  \\
%Large work items (too large to be completed by a single team in one iteration) whose description can contain values as high level requirements./epic
\textbf{\faEdit {} Persona:} state users values expectations in persona definition as goals to be satisfied by the system.& T &  \\
%reflects human personality and goals of a specific group of users that can be modified to capture and describe values people may hold.
\textbf{\faEdit {} User Journey Map:} describe the values of users affected by system usage when they try to achieve their goals.& T &  \\
%Visual descriptions of emotions a user goes through while accomplishing their goals that can be expanded to express values affected in fulfilling their goals through system use. & T &  \\
\textbf{\faLightbulbO{} Checklist:} list values to be considered during development and validated through users feedback of the system.& T &  \\
%list values to be considered during system development/evaluation to reduce failure due to potential limits of human memory or attention and also to ensure task completeness& 
%A job-aid artefact listing values to be considered during system development/evaluation to reduce failure due to potential limits of human memory or attention and ensures task completeness. & T \& P &  \\
\textbf{\faLightbulbO{} Legislative Requirement:} follow regulatory guidelines/standards to avoid violations of privacy/security etc.& P &  \\
%Regulations from government and consumer right protection bodies to ensure human values like privacy/security etc. are not violated by software.& P &  \\
\textbf{\faLightbulbO{} Corporate Directive:} introduce directives encouraging values consideration in software beyond security/privacy.& P &  \\ \hline
\multicolumn{3}{c}{\textbf{Roles}} \\ \hline
\textbf{\faEdit {} Product Owners:} optimise business value by ensuring human values are also addressed in the system delivered.& T &  \\
%optimises business value creation in the product and also ensure human values are delivered in the system. & T &  \\
\textbf{\faEdit {} Business Owners:} provide inputs on what satisfies users values expectations to maximise value for stakeholders.& T &  \\
%determines what maximises value creation for the stakeholders and also provides inputs as to what satisfies stakeholders' human value expectations. & T &  \\
\textbf{\faEdit {} Release Train Engineer:} ensure alignment between Agile and human values is never derailed during development.& T &  \\
%\textbf{\faEdit {} Release Train Engineer:} shepherds the delivery teams to ensure the alignment with (agile and) human values is never derailed throughout software development life-cycle. & T &  \\
\textbf{\faLightbulbO{} Value Champions:} actively advocate for values inclusion and keep it alive in people's minds to ensure success.& T &  \\
\textbf{\faLightbulbO{} Values Mentors:} guide development teams and encourage continuous adherence to values while developing software.& T &  \\
\textbf{\faLightbulbO{} Values Translators:} communicate values concepts in a terminology understandable for the development teams.& T &  \\
\textbf{\faLightbulbO{} Values Promoters:} advocate for inclusion of human values in software and help overcome barriers encountered.& T &  \\
\textbf{\faLightbulbO{} Value Officers:} answer values-specific questions and ensure values related directives and guidelines are adhered to.& T &  \\ \hline
\multicolumn{3}{c}{\textbf{Ceremonies}} \\ \hline
\textbf{\faEdit {} Stand-ups:} align development work with its `higher propose'; reflect on 'how \textit{this} work upholds \textit{that} human value'.& P &  \\
%can go beyond sharing work progress to align the development work with it's `higher propose' through questions like 'how is the work you are doing today upholding that value'& P &  \\
\textbf{\faEdit {} Review Meetings:} reflect on current practices and propose new ways to embed human values in software. & P &  \\
%facilitate  review  team  practices  to  identify  was  for  improvement  to  be  expanded  to  review activities and practices to embed values
\textbf{\faEdit {} Planning Meetings:} align organisational vision with stakeholder values to plan software delivery accordingly. & P &  \\
%help align all the teams to a shared vision to be modified to align  stakeholder value expectations with development organisation's values. & P &  \\
\textbf{\faEdit {} \textbf{Kick Offs:}} allow key stakeholders to define major human values objectives for the entire project. & P &  \\ \hline
%allow key stakeholders to define major project  goals and can also be used to define values objectives for the entire project. & P & 
\multicolumn{3}{c}{\textbf{Practices}} \\ \hline
\textbf{\faEdit {} Testing:} seek user feedback beyond usability, functionality to capture users experiences of their values expectations. & T &  \\
%seeking feedback beyond usability, functionality and performance to capture users experiences of their values expectations. & T &  \\
\faLightbulbO{} \textbf{Values Conversations:} prioritise human values and contemplate the implications of values breaches by software use.& T &  
%focus on discussing human values, contemplating the implications of values breaches and identifying ways to embed them into software delivery.& T &  
\\ \hline
\multicolumn{3}{c}{\textbf{ Culture}} \\ \hline
\textbf{\faUsers {} Hiring/Induction:} hire people with values aligned to the organisational values to foster a values-driven culture.& P &  \\
\textbf{\faUsers {} Leadership:} role-model values-based thinking and action as a behaviour for the development teams.& P &  \\
%that rubs off values-based thinking and action onto the development teams by role modelling it as a behaviour rather than seeking compliance through command and control.& P &  \\
\textbf{\faUsers {} Collective Responsibility:} share responsibility to address human values throughout the development life cycle.
& P & \\ \hline
\multicolumn{3}{c}{\faLightbulbO{}: new ideas emerged; \faEdit{}: modifying existing items; \faUsers{}: Culture; T: SAFe \textbf{Team} Level; P: SAFe \textbf{Program} Level} \\
\end{tabular}%
} \quad
\end{table*}

==> Tables/ValuesCategories.tex <==
\begin{table}[]
\centering
\caption{Value categories and descriptions [*]}
\label{tbl:valuescategories}
\resizebox{\linewidth}{!}{
{\renewcommand{\arraystretch}{1.15}
\begin{tabular}{p{2cm}l}
\hline
\textbf{Value Category} & \textbf{Description (motivational goals)}                                                                                                                              \\ \hline
\textbf{Self-direction}          & \begin{tabular}[c]{@{}l@{}}Independent thought and action–choosing, creating,\\ exploring\end{tabular}                                                                \\ \hline
\textbf{Stimulation}             & Excitement, novelty, and challenge in life                                                                                                                             \\ \hline
\textbf{Hedonism}                & Pleasure or sensuous gratification for oneself                                                                                                                         \\ \hline
\textbf{Achievement}             & \begin{tabular}[c]{@{}l@{}}Personal success through demonstrating competence \\ according to social standards\end{tabular}                                             \\ \hline
\textbf{Power}                   & \begin{tabular}[c]{@{}l@{}}Social status and prestige, control or dominance over\\ people and resources\end{tabular}                                                  \\ \hline
\textbf{Security}                & \begin{tabular}[c]{@{}l@{}}Safety, harmony, and stability of society, of relationships,\\ and of self\end{tabular}                                                    \\ \hline
\textbf{Conformity}              & \begin{tabular}[c]{@{}l@{}}Restraint of actions, inclinations, and impulses likely to upset\\ or harm others and violate social expectations or norms\end{tabular} \\ \hline
\textbf{Tradition}   & \begin{tabular}[c]{@{}l@{}}Respect, commitment, and acceptance of the customs/ ideas \\ that one’s culture or religion provides\end{tabular}                           \\ \hline
\textbf{Benevolence}             & \begin{tabular}[c]{@{}l@{}}Preserving and enhancing the welfare of those with whom one\\ is in frequent personal contact\end{tabular}                                  \\ \hline
\textbf{Universalism}            & \begin{tabular}[c]{@{}l@{}}Understanding, appreciation, tolerance, and protection for the \\ welfare of all people and for nature\end{tabular}                          \\ \hline
\end{tabular}
}
}\quad
\end{table}

==> sections/07-relatedWork.tex <==
\section{Related Work}
\subsection{Human Values in Software Development Process}
Human values are discussed as a part of technology design since the 1970's ~\cite{van2015design}.
\textit{Value Sensitive Design (VSD)} is recognised as one of the origins that embed social and moral values in technology development~\cite{van2015design}. To date, VSD has mainly been applied in human-computer interaction (HCI)~\cite{Davis2015}. Unfortunately, VSD is hardly adopted into day to day software development practices~\cite{aldewereld2015design}, despite a few isolated attempts to convert it as a part of SDLC~\cite{friedman2002value, van2015participatory}.

To the best of our knowledge, in the SE mainstream, there is no systematic approach that embeds human values into SDLC from start to finish, i.e., requirement elicitation to software delivery. However, a limited number of human values such as security, privacy and accessibility, has been studied in SE as software quality attributes \cite{whittle2019your}. Moreover, we recognise emerging studies in SE that attempts to incorporate human values into different parts of SDLC. 

\textit{Value-Based Requirement Engineering (VBRE)} uses stakeholders' values, motivations and emotions for eliciting value requirements and analysing soft issues of software~\cite{thew2018value}. By introducing \textit{Values-First SE}~\cite{ferrario2016values}, Ferrario and others attempt to give more visibility to the interplay between SE choices and underlying human values. In another study, Ferrario et al. introduce the~\textit{Values Q-sort} method that aims to measure developers' values in SE \cite{winter2018measuring}. Each of these techniques addresses one phase or specific consideration of the SDLC. Aldewereld and others attempt to cover all phases of SDLC with their~\textit{Value-Sensitive Software Development (VSSD)} conceptual framework~\cite{aldewereld2015design}, which considers a three-layer architecture to translate human values into software features. However, all of these studies are either at a conceptual level or need to go through industrial-level trials before they become a part of the everyday practice of software engineers. 

% \subsection{Human Values in Software Development Process}
% \begin{itemize}
%     \item Values are known in RE an early design phases (cite VBRE, VSD), but did not correctly transform through out the SDLC.
%     \item A few noteworthy attempts, Values-first SE, VSSD and other.
%     \item agile as one of the methods that includes a part of these values like value to customer
% \end{itemize}
% \subsection{Values in Agile}

% \begin{itemize}

%     \item agile methods such as Scrum mainly talk about business value, quote examples from Scrum  Primer/Guide
%     \item define business value as applied in agile/scrum
%     \item summarize what human values, if any, are addressed in agile/scrum directly or indirectly
%     \item motivate why its important to address/embed human values in agile processes such as Scrum and essential SAFe + fact that there are no studies that do this, ours is a first
% \end{itemize}
\subsection{Human Values and Agile Methods}

Miller and Larson\cite{miller2005agile} argued that human values and ethical principles should be the backbone of evaluating Agile methods. They suggested two ethical analysis techniques for this purpose: \textit{utilitarian analysis} and \textit{deontological analysis}. The former helps software engineers understand and analyse the potential consequences of their actions and decisions on the stakeholders who are directly and indirectly affected by the software. The latter focuses on the intentions of software engineers and encourages them to consider human values and human needs as the leading driver in their decisions. Several studies have attempted to extend or augment Agile methods to put the needs and constraints of customers and end-users at the centre of the software development process, particularly at the design phase\cite{brhel2015exploring},\cite{schon2017agile}. In an extensive investigation of literature, Schön et al.\cite{schon2017agile} highlighted Human-Centered Design, Design Thinking, Contextual Inquiry, and Participatory Design as prominent approaches used in Agile software development for this purpose. However, these methods mainly focus on the business values of customers and end users and are less concerned, if at all, with human values. 

More recent works have attempted to address human values in agile software development. Detweiler and Harbers\cite{detweiler2014value} proposed the idea of Value Stories Workshop to guide Agile teams in identifying and analysing what a system’s stakeholders consider as important in their daily life (i.e., human values). Fagerholm and Pagels\cite{fagerholm2014examining} explored the values of developers working in the context of Lean and Agile and compared them with the basic human values (i.e., the Schwartz values). The study shows that Lean and Agile values, can be organised into 11 groups (e.g., “the freedom to organise” and “collaboration”). Fagerholm and Pagels observed that Lean and Agile values (e.g., “reliance on people”) and the basic human values (e.g., “benevolence”) are contented, but they are not equal. In another study\cite{lawrence2012interpretation}, Lawrence and Rodriguez analysed two sources of Agile documentation (i.e., the vendor-sponsored whitepapers and IT and business magazine articles) to understand how basic values in the Lasswell value framework are interpreted and expressed by Agile community. The Lasswell value framework includes eight values: power, respect, rectitude, affection, well-being, wealth, skill, and enlightenment. The study found that power, enlightenment, wealth, and skill are the most frequently expressed values among the contributors to the Agile method. However, the level of correlation of these four strong values to the values expressed in the Agile Manifesto is different. Enlightenment and skill are highly correlated to the Agile Manifesto, while wealth and power are not explicitly mapped to the values in the Agile Manifesto. It was also observed that rectitude, respect, affection, and well-being were less expressed. 

To the best of our knowledge, we are the first to investigate the need for human values across the entire agile process framework, in particular, in the SAFe model. 







